A Systematic Mapping Study of Digital Twins for Diagnosis in Transportation

In recent years, digital twins have been proposed and implemented in various fields with potential applications ranging from prototyping to maintenance. Going forward, they are to enable numerous efficient and sustainable technologies, among them autonomous cars. However, despite a large body of research in many fields, academics have yet to agree on what exactly a digital twin is -- and as a result, what its capabilities and limitations might be. To further our understanding, we explore the capabilities of digital twins concerning diagnosis in the field of transportation. We conduct a systematic mapping study including digital twins of vehicles and their components, as well as transportation infrastructure. We discovered that few papers on digital twins describe any diagnostic process. Furthermore, most existing approaches appear limited to system monitoring or fault detection. These findings suggest that we need more research for diagnostic reasoning utilizing digital twins.

==> data/applications/bridge.tex <==
bridge~\mbox{\cite{dang2018digital}} & predict future performance \\
bridge~\mbox{\cite{forstner2019automated}} & detect structural damage \\
cable-supported bridge~\mbox{\cite{shim2019digital}} & provide real-time assessment of bridge behaviour \\
bridge~\mbox{\cite{ye2019digital}} & improve structural health monitoring, improve whole-life management \\
bridge~\mbox{\cite{bittencourt2021digital}} & real-time risk evaluation \\
girder bridge~\mbox{\cite{dang2020bridge}} & enable preventive maintenance \\
suspension bridge~\mbox{\cite{dang2020master}} & continuously analyse stability, estimate actual bridge behaviour \\
Mohammed VI bridge~\mbox{\cite{sofia2020mobile}} & inspect surface distortions \\
highway bridge~\mbox{\cite{ye2020technology}} & capture critical behaviour, identify root causes of deficiencies \\
bridge~\mbox{\cite{bhouri2021model}} & detect cracks \\
bridge group~\mbox{\cite{dan2021digital}} & provide early safety warnings \\
bridge~\mbox{\cite{kang2021multimedia}} & predict optimal time for maintenance, reduce maintenance costs, extend bridge lifespan \\
bridge steel deck, traffic load~\mbox{\cite{yu2022digital}} & evaluate fatigue, predict remaining life \\
bridge~\mbox{\cite{zhao2022developing}} & predict bridge behaviour under random traffic


==> data/applications/component_other.tex <==
automotive braking system~\mbox{\cite{magargle2017simulation}} & analyze failure data, train predictive maintenance analytics \\
planetary transmissions~\mbox{\cite{algin2018models}} & calculate dependability, calculate lifetime \\
brake pad~\mbox{\cite{rajesh2019digital}} & estimate brake wear, enable predictive maintenance \\
electric propulsion drive system~\mbox{\cite{rassõlkin2019digital}} & none \\
electric vehicle motor~\mbox{\cite{venkatesan2019health}} & estimate remaining useful life \\
automated braking systems~\mbox{\cite{dygalo2020monitoring,dygalo2020real}} & diagnose internal faults \\
electric vehicle powertrains~\mbox{\cite{rodríguez2021thermal}} & estimate thermal parameters, estimate system state \\
supercapacitor~\mbox{\cite{yang2021supercapacitor}} & estimate state of charge, estimate state of health


==> data/applications/people.tex <==
vehicle, driver~\mbox{\cite{kumar2018novel}} & predict driver intentions, predict traffic chaos \\
passengers, public transport vehicles~\mbox{\cite{amrani2020architecture}} & predict passenger flow, estimate incident durations \\
passengers, public transport vehicles~\mbox{\cite{campolo2020digital}} &  collect valuable data  \\
vehicles, drivers, pedestrians~\mbox{\cite{liu2020sensor}} & predict driver intentions, avoid accidents \\
vehicles, drivers~\mbox{\cite{wang2020digital}} & cooperative ramp merging \\
pedestrians, cyclists, bike rental stores~\mbox{\cite{clemen2021multi,lenfers2021improving}} & provide stakeholders with reliable information \\
vehicles, pedestrians, obstacles~\mbox{\cite{guo2021digital}} & visualize traffic \\
vehicles, people~\mbox{\cite{marai2021roads}} & enable autonomous vehicles, diminish crime, help insurance companies resolve conflicts \\
virtual people, virtual cars, virtual traffic lights~\mbox{\cite{yun2021virtualization}} & enable autonomous vehicles \\
pedestrians, cyclists, cars, traffic infrastructure~\mbox{\cite{ma2022virtual}} & identify potential crashes, emit warning signals \\
human beings, vehicles, traffic~\mbox{\cite{wang2022mobility}} & predict driver behaviour, detect driver anomalies, predict component failure, traffic flow monitoring for variable speed limits


==> data/applications/road.tex <==
roads~\mbox{\cite{machl2019planning}} & determine road use, determine road load \\
road surface, vehicles~\mbox{\cite{naets2019approach}} & identify vehicle parameters, identify road geometry \\
road~\mbox{\cite{meža2021digital}} & monitor structural health \\
road pavements~\mbox{\cite{damico2022integrating}} & detect pavement distress, determine drainage basins \\
road~\mbox{\cite{han2022bim}} & monitor compaction quality


==> data/applications/traffic.tex <==
traffic noise~\mbox{\cite{radenkovic2020iot}} & predict noise levels \\
traffic environment~\mbox{\cite{tihanyi2021towards}} & detect pedestrians \\
road traffic~\mbox{\cite{wild2021joint}} & detect vehicles, detect pedestrians \\
virtual people, virtual cars, virtual traffic lights~\mbox{\cite{yun2021virtualization}} & enable autonomous vehicles \\
traffic~\mbox{\cite{hu2022digital}} & estimate speed and volume \\
pedestrians, cyclists, cars, traffic infrastructure~\mbox{\cite{ma2022virtual}} & identify potential crashes, emit warning signals \\
human beings, vehicles, traffic~\mbox{\cite{wang2022mobility}} & predict driver behaviour, detect driver anomalies, predict component failure, traffic flow monitoring for variable speed limits \\
vehicles, traffic~\mbox{\cite{xu2022developing}} & propose eco-routing strategies, mitigate carbon emissions \\
bridge steel deck, traffic load~\mbox{\cite{yu2022digital}} & evaluate fatigue, predict remaining life


==> data/stats.tex <==
% DO NOT EDIT stats.tex DIRECTLY!  IT IS AUTOMATICALLY GENERATED AND
% YOUR CHANGES WILL BE LOST WITH THE NEXT UPDATE!  TO PRESERVE YOUR
% CHANGES, EDIT stats.tex.in INSTEAD.

% When adding new statistics, the layout below should be followed, i.e
% one block per table, square brackets to denote access (similar to C,
% C++, or Python), with the \@nameuse def'd on top and the \@namedefs
% following.
% To get the statistics themselves, three curly braces are to be used
% -- one for TeX, two for recfmt.  This style is unsupported in version
% 1.8 of GNU Recutils (the latest release as of time of writing),
% but a patch to add it has already been accepted upstream.

\makeatletter
\RequirePackage{fmtcount}

\def\total[#1]{\@nameuse{total@#1}}
\def\totalN[#1]{\numberstringnum{\total[#1]}}
\def\TotalN[#1]{\Numberstringnum{\total[#1]}}
\def\totaldef[#1]#2{\@namedef{total@#1}{#2}}

\def\subject[#1]{\@nameuse{subject@#1}}
\def\subjectN[#1]{\numberstringnum{\subject[#1]}}
\def\SubjectN[#1]{\Numberstringnum{\subject[#1]}}
\def\subject@def[#1]#2{\@namedef{subject@#1}{#2}}

\def\method[#1]{\@nameuse{method@#1}}
\def\methodN[#1]{\numberstringnum{\method[#1]}}
\def\MethodN[#1]{\Numberstringnum{\method[#1]}}
\def\method@def[#1]#2{\@namedef{method@#1}{#2}}

\def\storage[#1]{\@nameuse{storage@#1}}
\def\storageN[#1]{\numberstringnum{\storage[#1]}}
\def\StorageN[#1]{\Numberstringnum{\storage[#1]}}
\def\storage@def[#1]#2{\@namedef{storage@#1}{#2}}

\def\lifecycle[#1]{\@nameuse{lifecycle@#1}}
\def\lifecycleN[#1]{\numberstringnum{\lifecycle[#1]}}
\def\LifecycleN[#1]{\Numberstringnum{\lifecycle[#1]}}
\def\lifecycle@def[#1]#2{\@namedef{lifecycle@#1}{#2}}

\def\step[#1]{\@nameuse{step@#1}}
\def\stepN[#1]{\numberstringnum{\step[#1]}}
\def\StepN[#1]{\Numberstringnum{\step[#1]}}
\def\step@def[#1]#2{\@namedef{step@#1}{#2}}

\def\model[#1]{\@nameuse{model@#1}}
\def\modelN[#1]{\numberstringnum{\model[#1]}}
\def\ModelN[#1]{\Numberstringnum{\model[#1]}}
\def\model@def[#1]#2{\@namedef{model@#1}{#2}}

\def\byyear[#1]{\@nameuse{byyear@#1}}
\def\byyearN[#1]{\numberstringnum{\byyear[#1]}}
\def\ByyearN[#1]{\Numberstringnum{\byyear[#1]}}
\def\byyear@def[#1]#2{\@namedef{byyear@#1}{#2}}

\totaldef[records]{88}
\totaldef[papers]{90}
\totaldef[infosec statements]{15}

\totaldef[records]{88}
\totaldef[papers]{90}
\totaldef[infosec statements]{15}

\subject@def[component]{24}
\subject@def[environment]{43}
\subject@def[people]{9}
\subject@def[vehicle]{27}

\method@def[artificial intelligence]{32}
\method@def[machine learning]{30}
\method@def[numerical analysis]{20}
\method@def[simulation and visualization]{20}
\method@def[signal processing]{13}
\method@def[fault trees]{2}
\method@def[thresholds]{4}
\method@def[other]{12}
\method@def[unknown]{10}

\storage@def[device]{7}
\storage@def[database]{7}
\storage@def[edge]{12}
\storage@def[fog]{1}
\storage@def[cloud]{33}
\storage@def[blockchain]{3}
\storage@def[edge and cloud]{9}
\storage@def[unknown]{37}

\lifecycle@def[prototype]{9}
\lifecycle@def[in use]{85}
\lifecycle@def[postmortem]{4}

\step@def[monitoring]{54}
\step@def[detection]{32}
\step@def[localization]{8}
\step@def[mitigation]{8}

\model@def[finite element]{12}
\model@def[building info]{8}
\model@def[equivalent circuit]{10}
\model@def[hidden markov]{1}
\model@def[mass spring damper]{1}
\model@def[doyle fuller newman]{2}
\model@def[lumped thermal]{2}
\model@def[agent based]{2}
\model@def[behavioural]{15}
\model@def[behavioural aggregated]{17}
\model@def[structural]{3}
\model@def[geometric]{18}
\model@def[geometric aggregated]{26}
\model@def[statistical]{5}
\model@def[statistical aggregated]{6}
\model@def[mathematical]{7}
\model@def[mathematical aggregated]{19}
\model@def[physics]{13}
\model@def[physics aggregated]{25}
\model@def[data]{22}
\model@def[phenomenological]{0}

\byyear@def[2017]{1}
\byyear@def[2018]{6}
\byyear@def[2019]{10}
\byyear@def[2020]{16}
\byyear@def[2021]{40}
\byyear@def[2022]{15}

\makeatother


==> data/stats2.tex <==
\makeatletter
\step@def[environment monitoring]{25}
\step@def[environment detection]{18}
\step@def[environment localization]{3}
\step@def[environment mitigation]{2}

\step@def[component monitoring]{19}
\step@def[component detection]{5}
\step@def[component localization]{2}
\step@def[component mitigation]{0}

\step@def[people monitoring]{7}
\step@def[people detection]{3}
\step@def[people localization]{1}
\step@def[people mitigation]{1}

\step@def[vehicle monitoring]{15}
\step@def[vehicle detection]{11}
\step@def[vehicle localization]{4}
\step@def[vehicle mitigation]{5}

\model@def[environment geometric aggregated]{19}
\model@def[environment behavioural aggregated]{8}
\model@def[environment physics aggregated]{6}
\model@def[environment statistical aggregated]{2}
\model@def[environment mathematical aggregated]{11}
\model@def[environment data]{14}

\model@def[component geometric aggregated]{1}
\model@def[component behavioural aggregated]{1}
\model@def[component physics aggregated]{16}
\model@def[component statistical aggregated]{1}
\model@def[component mathematical aggregated]{4}
\model@def[component data]{4}

\model@def[vehicle geometric aggregated]{9}
\model@def[vehicle behavioural aggregated]{11}
\model@def[vehicle physics aggregated]{5}
\model@def[vehicle statistical aggregated]{3}
\model@def[vehicle mathematical aggregated]{3}
\model@def[vehicle data]{5}

\model@def[people geometric aggregated]{4}
\model@def[people behavioural aggregated]{7}
\model@def[people physics aggregated]{0}
\model@def[people statistical aggregated]{1}
\model@def[people mathematical aggregated]{0}
\model@def[people data]{2}

\totaldef[environment infosec statements]{7}
\totaldef[component infosec statements]{2}
\totaldef[people infosec statements]{4}
\totaldef[vehicle infosec statements]{7}

\method@def[environment artificial intelligence]{19}
\method@def[environment machine learning]{17}
\method@def[environment numerical analysis]{7}
\method@def[environment simulation and visualization]{13}
\method@def[environment signal processing]{7}
\method@def[environment fault trees]{1}
\method@def[environment thresholds]{2}
\method@def[environment other]{6}
\method@def[environment unknown]{5}

\method@def[component artificial intelligence]{5}
\method@def[component machine learning]{5}
\method@def[component numerical analysis]{11}
\method@def[component simulation and visualization]{3}
\method@def[component signal processing]{2}
\method@def[component fault trees]{0}
\method@def[component thresholds]{1}
\method@def[component other]{1}
\method@def[component unknown]{3}

\method@def[people artificial intelligence]{7}
\method@def[people machine learning]{7}
\method@def[people numerical analysis]{0}
\method@def[people simulation and visualization]{1}
\method@def[people signal processing]{1}
\method@def[people fault trees]{0}
\method@def[people thresholds]{0}
\method@def[people other]{1}
\method@def[people unknown]{1}

\method@def[vehicle artificial intelligence]{11}
\method@def[vehicle machine learning]{11}
\method@def[vehicle numerical analysis]{3}
\method@def[vehicle simulation and visualization]{6}
\method@def[vehicle signal processing]{5}
\method@def[vehicle fault trees]{0}
\method@def[vehicle thresholds]{2}
\method@def[vehicle other]{4}
\method@def[vehicle unknown]{2}

\totaldef[environment records]{43}
\totaldef[component records]{24}
\totaldef[people records]{9}
\totaldef[vehicle records]{27}

\storage@def[environment unknown]{24}
\storage@def[environment device]{1}
\storage@def[environment database]{5}
\storage@def[environment edge]{4}
\storage@def[environment fog]{0}
\storage@def[environment cloud]{12}
\storage@def[environment blockchain]{1}

\storage@def[component unknown]{6}
\storage@def[component device]{6}
\storage@def[component database]{1}
\storage@def[component edge]{2}
\storage@def[component fog]{0}
\storage@def[component cloud]{11}
\storage@def[component blockchain]{0}

\storage@def[vehicle unknown]{9}
\storage@def[vehicle device]{1}
\storage@def[vehicle database]{2}
\storage@def[vehicle edge]{7}
\storage@def[vehicle fog]{1}
\storage@def[vehicle cloud]{13}
\storage@def[vehicle blockchain]{2}

\storage@def[people unknown]{2}
\storage@def[people device]{0}
\storage@def[people database]{0}
\storage@def[people edge]{3}
\storage@def[people fog]{1}
\storage@def[people cloud]{7}
\storage@def[people blockchain]{1}


\makeatother

